AppSlice: A system for application-centric design of 5G and edge computing applications

Applications that use edge computing and 5G to improve response times consume both compute and network resources. However, 5G networks manage only network resources without considering the application's compute requirements, and container orchestration frameworks manage only compute resources without considering the application's network requirements. We observe that there is a complex coupling between an application's compute and network usage, which can be leveraged to improve application performance and resource utilization. We propose a new, declarative abstraction called AppSlice that jointly considers the application's compute and network requirements. This abstraction leverages container management systems to manage edge computing resources, and 5G network stacks to manage network resources, while the joint consideration of coupling between compute and network usage is explicitly managed by a new runtime system, which delivers the declarative semantics of the app slice. The runtime system also jointly manages the edge compute and network resource usage automatically across different edge computing environments and 5G networks by using two adaptive algorithms. We implement a complex, real-world, real-time monitoring application using the proposed app slice abstraction, and demonstrate on a private 5G/LTE testbed that the proposed runtime system significantly improves the application performance and resource usage when compared with the case where the coupling between the compute and network resource usage is ignored.

==> files/dataset.tex <==
\subsection{Dataset}
\lSec{dataset}
We used \textit{Labelled movie trailer dataset (LMTD)} \cite{10.1016/j.asoc.2017.08.029} for our experiments. We selected a video sequence containing 22 unique people from this dataset and used it as input video feed. 10 among the 22 were pre-registered in ``Biometrics manager". 

%We then ran real-time monitoring application under various conditions and checked if these 10 individuals were correctly recognized or not across various experiments.


==> files/ref.tex <==
% Generated by IEEEtran.bst, version: 1.14 (2015/08/26)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{cao_overview_2020}
\BIBentryALTinterwordspacing
K.~Cao, Y.~Liu, G.~Meng, and Q.~Sun, ``An {Overview} on {Edge} {Computing}
  {Research},'' \emph{IEEE Access}, vol.~8, pp. 85\,714--85\,728, 2020.
  [Online]. Available: \url{https://ieeexplore.ieee.org/document/9083958/}
\BIBentrySTDinterwordspacing

\bibitem{9345798}
M.~H.~C. Garcia, A.~Molina-Galan, M.~Boban, J.~Gozalvez, B.~Coll-Perales,
  T.~Şahin, and A.~Kousaridas, ``A tutorial on {5G} nr v2x communications,''
  \emph{IEEE Communications Surveys Tutorials}, pp. 1--1, 2021.

\bibitem{mec-netslice}
A.~Ksentini and P.~A. Frangoudis, ``Toward slicing-enabled multi-access edge
  computing in 5g,'' \emph{IEEE Network}, vol.~34, no.~2, pp. 99--105, 2020.

\bibitem{aws-verizon-5g}
\BIBentryALTinterwordspacing
``Transformational performance with 5{G} and edge computing.'' [Online].
  Available:
  \url{https://d1.awsstatic.com/Wavelength2020/AWS-5G-edge-Infographic-FINAL-Aug2020-2.pdf}
\BIBentrySTDinterwordspacing

\bibitem{edge-computing-in-5g}
N.~Hassan, K.-L. Yau, and C.~Wu, ``Edge computing in 5{G}: A review,''
  \emph{IEEE Access}, vol.~PP, pp. 1--1, 08 2019.

\bibitem{8845282}
N.~Huin, P.~Medagliani, S.~Martin, J.~Leguay, L.~Shi, S.~Cai, J.~Xu, and
  H.~Shi, ``Hard-isolation for network slicing,'' in \emph{IEEE INFOCOM 2019 -
  IEEE Conf. on Computer Communications Workshops (INFOCOM WKSHPS)}, 2019, pp.
  955--956.

\bibitem{demystifying-network-slicing}
\BIBentryALTinterwordspacing
``Demystifying network slicing.'' [Online]. Available:
  \url{https://ribboncommunications.com/sites/default/files/2020-05/Demystifying-Network-Slicing-WP.pdf}
\BIBentrySTDinterwordspacing

\bibitem{9382385}
S.~Wijethilaka and M.~Liyanage, ``Survey on network slicing for {I}nternet of
  {T}hings realization in {5G} networks,'' \emph{IEEE Communications Surveys
  Tutorials}, pp. 1--1, 2021.

\bibitem{9272281}
A.~Banchs, G.~de~Veciana, V.~Sciancalepore, and X.~Costa-Perez, ``Resource
  allocation for network slicing in mobile networks,'' \emph{IEEE Access},
  vol.~8, pp. 214\,696--214\,706, 2020.

\bibitem{kubernetes-link}
\BIBentryALTinterwordspacing
``Kubernetes.'' [Online]. Available: \url{https://kubernetes.io/}
\BIBentrySTDinterwordspacing

\bibitem{celona-link}
\BIBentryALTinterwordspacing
``Celona.'' [Online]. Available: \url{https://celona.io/}
\BIBentrySTDinterwordspacing

\bibitem{iperf3}
\BIBentryALTinterwordspacing
``i{P}erf.'' [Online]. Available: \url{https://iperf.fr/iperf-doc.php}
\BIBentrySTDinterwordspacing

\bibitem{multitech-link}
\BIBentryALTinterwordspacing
``Multitech.'' [Online]. Available:
  \url{https://www.multitech.com/brands/multiconnect-ecell}
\BIBentrySTDinterwordspacing

\bibitem{7901477}
T.~X. Tran, A.~Hajisami, P.~Pandey, and D.~Pompili, ``Collaborative mobile edge
  computing in {5G} networks: New paradigms, scenarios, and challenges,''
  \emph{IEEE $Comm^{ns}$ Magazine}, vol.~55, no.~4, pp. 54--61, 2017.

\bibitem{10.1016/j.asoc.2017.08.029}
J.~Wehrmann, ``Movie genre classification: A multi-label approach based on
  convolutions through time,'' \emph{Applied Soft Computing}, vol.~61, 2017.

\bibitem{7877341}
H.~A. Ismail and M.~Riasetiawan, ``Cpu and memory performance analysis on
  dynamic and dedicated resource allocation using xenserver in data center
  environment,'' in \emph{2016 2nd International Conf. on Science and
  Technology-Computer (ICST)}, 2016, pp. 17--22.

\bibitem{tosca}
\BIBentryALTinterwordspacing
``Topology and orchestration specification for cloud applications version
  1.0,'' November, 2013, {OASIS} {S}tandard. [Online]. Available:
  \url{http://docs.oasis-open.org/tosca/TOSCA/v1.0/TOSCA-v1.0.html}
\BIBentrySTDinterwordspacing

\bibitem{9389979}
R.~Liu, X.~Hai, S.~Du, L.~Zeng, J.~Bai, and J.~Liu, ``Application of {5G}
  network slicing technology in smart grid,'' in \emph{2021 IEEE 2nd
  International Conf. on Big Data, Artificial Intelligence and Internet of
  Things Engineering (ICBAIE)}, 2021, pp. 740--743.

\bibitem{9152315}
W.~Li, R.~Liu, Y.~Dai, D.~Wang, H.~Cai, J.~Fan, and Y.~Li, ``Research on
  network slicing for smart grid,'' in \emph{2020 IEEE 10th International Conf.
  on Electronics Information and Emergency Communication (ICEIEC)}, 2020, pp.
  107--110.

\bibitem{10.1109/MNET.011.1900458}
A.~Vergutz, G.~Noubir, and M.~Nogueira, ``Reliability for smart healthcare: A
  network slicing perspective,'' \emph{IEEE Network}, vol.~34, pp. 91--97, 07
  2020.

\bibitem{li2016endtoend}
\BIBentryALTinterwordspacing
Q.~Li, G.~Wu, A.~Papathanassiou, and U.~Mukherjee, ``An end-to-end network
  slicing framework for {5G} wireless communication systems,'' 2016. [Online].
  Available: \url{https://arxiv.org/pdf/1608.00572.pdf}
\BIBentrySTDinterwordspacing

\end{thebibliography}

